Recipe for higher-order topology on the triangular lattice

We present a recipe for an electronic 2D higher order topological insulator (HOTI) on the triangular lattice that can be realized in a large family of materials. The essential ingredient is mirror symmetry breaking, which allows for a finite quadrupole moment and trivial $\mathbb{Z}_2$ index. The competition between spin-orbit coupling and the symmetry breaking terms gives rise to four topologically distinct phases; the HOTI phase appears when symmetry breaking dominates, including in the absence of spin-orbit coupling. We identify triangular monolayer adsorbate systems on the (111) surface of zincblende/diamond type substrates as ideal material platforms and predict the HOTI phase for $X=$(Al,B,Ga) on SiC.

==> methods_0.tex <==
\section{Methods}

\small{\noindent\textbf{DFT calculations}}\newline
\footnotesize{For our theoretical study of XXX on SiC(0001) we employed state-of-the-art first-principles calculations based on the density functional theory as implemented in the \ac{VASP} \cite{VASP1}, within the \ac{PAW} method \cite{VASP2,PAW}. For the exchange-correlation potential the PBE functional was used \cite{PBE}, by expanding the Kohn-Sham wave functions into plane-waves up to an energy cut-off of XXX eV. For the bulk calculations, we sampled the Brillouin zone on an $X\timesX\times1$ regular mesh, and when considered, \ac{SOC} was self-consistently included \cite{SOC_VASP}\pe{No SOC so far}. 
%\ac{OAM} expectation values and
We consider a $(1\times1)$ reconstruction of triangular XXX on XXX layers of Si-terminated SiC(0001) with an in-plane lattice constant of $3.07\,\text{\AA}$. The equilibrium structure is obtained by relaxing all atoms until all forces converged below $0.005\,\text{eV/\AA}$ resulting in an XXX-SiC distance of $d_{XXX-SiC}=XXX\,\text{\AA}$. To disentangle the electronic states of both surfaces a vacuum distance of at least XXX $\text{\AA}$ between periodic replicas in $z$-direction is assumed and the dangling bonds of the substrate terminated surface are saturated by hydrogen.}




